Probabilistically Robust Recourse: Navigating the Trade-offs between Costs and Robustness in Algorithmic Recourse

As machine learning models are increasingly being employed to make consequential decisions in real-world settings, it becomes critical to ensure that individuals who are adversely impacted (e.g., loan denied) by the predictions of these models are provided with a means for recourse. While several approaches have been proposed to construct recourses for affected individuals, the recourses output by these methods either achieve low costs (i.e., ease-of-implementation) or robustness to small perturbations (i.e., noisy implementations of recourses), but not both due to the inherent trade-offs between the recourse costs and robustness. Furthermore, prior approaches do not provide end users with any agency over navigating the aforementioned trade-offs. In this work, we address the above challenges by proposing the first algorithmic framework which enables users to effectively manage the recourse cost vs. robustness trade-offs. More specifically, our framework Probabilistically ROBust rEcourse (\texttt{PROBE}) lets users choose the probability with which a recourse could get invalidated (recourse invalidation rate) if small changes are made to the recourse i.e., the recourse is implemented somewhat noisily. To this end, we propose a novel objective function which simultaneously minimizes the gap between the achieved (resulting) and desired recourse invalidation rates, minimizes recourse costs, and also ensures that the resulting recourse achieves a positive model prediction. We develop novel theoretical results to characterize the recourse invalidation rates corresponding to any given instance w.r.t. different classes of underlying models (e.g., linear models, tree based models etc.), and leverage these results to efficiently optimize the proposed objective. Experimental evaluation with multiple real world datasets demonstrates the efficacy of the proposed framework.

==> section0.tex <==
As machine learning models are increasingly being deployed in high-stakes applications, there has been growing interest in providing recourse to individuals adversely impacted by model predictions (e.g., an applicant whose loan has been denied). To this end, several post hoc techniques have been proposed in recent literature. These techniques generate recourses under the assumption that the affected individuals will implement the prescribed recourses \emph{exactly}. However, recent studies suggest that individuals often implement recourses in a noisy and inconsistent manner -- 
e.g., raising their salary by \$505 if the prescribed recourse suggested an increase of \$500. Motivated by this, we introduce and study the problem of recourse invalidation in the face of noisy human responses. More specifically, we theoretically and empirically analyze the behavior of state-of-the-art algorithms, and demonstrate that the recourses generated by these algorithms are very likely to be invalidated if small changes are made to them. 
%in the case where recourses are implemented in a noisy manner. Our results demonstrate that the recourses provided by these algorithms become invalidated with a very high probability when . 
We further propose a novel framework, EXPECTing noisy responses (\texttt{EXPECT}), which addresses the aforementioned problem by explicitly minimizing the probability of recourse invalidation in the face of noisy responses. Experimental evaluation with multiple real world datasets demonstrates the efficacy of the proposed framework, and supports our theoretical findings. 
\hideh{
As machine learning (ML) models become more widely deployed in high-stakes applications,
counterfactual explanations have emerged as key tools for providing actionable model explanations
in practice. 
These techniques generate recourses under the assumption that the individual, for which recourse is computed, will respond accurately, i.e., the individual will make a `\emph{precision landing}' on the recourse suggestion. 
Motivated by evidence from real-world field experiments and empirical results, we study the problem of recourse invalidation under human response inaccuracies.
We do so by analyzing the recourse invalidation probability in the presence of random human response inaccuracies providing conditions when recourse is expected to be robust. 
We then derive upper bounds on the recourse invalidation probability which depend on general sparsity principles that are thought to be desirable for interpretable and actionable recourses.
To address the recourse invalidation problem algorithmically, we propose a new framework, EXPecting rEcourse unCerTainity (\texttt{EXPECT}), that explicitly incorporates a worst-case recourse invalidation target into the recourse objective to find robust recourses in the face of human response inconsistencies.}
